Deep Learning Service for Efficient Data Distribution Aware Sorting

In this paper, we present a neural network-enabled data distribution aware sorting method, coined as NN-sort. Our approach explores the potential of developing deep learning techniques to speed up large-scale sort operations, enabling data distribution aware sorting as a deep learning service. Compared to traditional pairwise comparison-based sorting algorithms, which sort data elements by performing pairwise operations, NN-sort leverages the neural network model to learn the data distribution and uses it to map large-scale data elements into ordered ones. Our experiments demonstrate the significant advantage of using NN-sort. Measurements on both synthetic and real-world datasets show that NN-sort yields 2.18x to 10x performance improvement over traditional sorting algorithms.

==> sec-background.tex <==
%\vspace{-0.7ex}
%%%%%%%% Section 2 %%%%%%%%
\section{Preliminaries}
\label{sec-background}
%\vspace{-0.7ex}
We first review notations for ER, blocking, and GPUs.



\stitle{Relations.}
Consider a relation schema $R =
(\eid, A_1, \dotsc, \allowbreak A_n)$, where $A_i$
is an attribute ($i\in[1,n]$), and \eid is an entity id, such that
each tuple of $R$ represents an entity with identity \eid.
A relation $D$ of $R$ is a set of tuples of schema $R$.


\stitle{Entity resolution.}
Given a relation $D$, ER is to identify all tuple pairs in $D$ that refer to the same real-life entity.
%Entity resolution aims at finding all matching entities within an entity collection or across two entity collections.
%Formally, an ER task receives as input an entity collection $\E$ and produces as output the set of all
%pairs of matching entity profiles within $\E$, \ie $\D(\E) = \{ (t, s):t\in \E , s\in \E, t = s\}$.
It returns a set of tuple pairs $(t_1, t_2)$ of $D$
that are identified
as {\em matches}. 
If $t_1$ does not match $t_2$, $(t_1, t_2)$
  is referred to as a \emph{mismatch}. 





\vspace{0.6ex}
Most existing methods typically conduct ER in three steps:

\etitle{(1) Data partitioning.}
The tuples in  relation $D$ are divided into multiple disjoint data partitions,
namely $P_1,P_2,..., P_m$,
so that tuples of similar entities are put into the same data partition.

\etitle{(2) Blocking.}
Each tuple pair $(t_1, t_2) $ from the same data partition $P$ (\ie $(t_1, t_2) \in P \times P$) is a potential match
that requires further verification.
To reduce the verification cost,
a blocking method $\A_\kw{block}$ is often adopted to filter out those pairs 
that are definitely mismatches \emph{efficiently}, 
instead of directly examining every tuple pair in $P \times P$.
Denote the resulting set of remaining tuple pairs obtained from  partition $P$ by $\kw{Ca}(P) = \{(t_1, t_2) \in P \times P \mid (t_1, t_2) \text{ is not filtered by } \A_\kw{block}\}$.

\etitle{(3) Matching.}
For the remaining tuple pairs in $\kw{Ca}(P)$ of each data partition $P$,
an accurate (but expensive) matcher will be applied,  to make the final decision of matches/mismatches.
%The final set of matches is $\kw{Ca}(D) = \cup_{i=1}^m \kw{Ca}(P_i)$.


\eat{
A candidate selection step often been split into two different
but related phrase: data partitioning and blocking. 
Data partitioning attempt to 
clusters similar entities into a
block collection $\B=\{B_1,B_2,...\}$ such that $\cup_{P\in\B}{P} = \E$.
Given an entity collection $\E$, a  function $f:\E\times\E\to\mathbb{B}$, 
blocking identifies all pairs of entity profiles in $\E$ 
that have $f$ return ture, \ie $\kw{Ca}(\E) = \{ (t,s)\in \E\Join\E, f(t,s) = true, t \neq s \}$.
}


\vspace{0.6ex}
Note that in some works, both steps (1) and (2) are called blocking.
To avoid ambiguity,
we follow~\cite{DeepBlocking}
and distinguish data partitioning from blocking.
The main focus of this work is the blocking step, whose goal is to design a method $\A_\kw{block}$ to output the set $\kw{Ca}(P)$ of candidate tuple pairs given a partition $P$.
Our work can be applied on the data partitions generated by \emph{any} existing data partitioning method.
Nevertheless,
we also optimize over multiple data partitions,
by exploiting designated GPU acceleration techniques (see Section~\ref{subsec:GPUs}).  

\revise{
While blocking focuses more on the efficiency and  matching focuses more on the accuracy,
they can be used without each other,
\eg one can directly employ rules~\cite{fan2011dynamic} for ER or
 apply an ER matcher~\cite{ditto} on the Cartesian product of the data.
In Section~\ref{sec-expt},
we tested \Hyper with/without a matcher,
to elaborate the trade-off between efficiency and accuracy.
\looseness=-1

}

\stitle{Blocking Problem.}
Formally, the problem is stated as follows.
\begin{itemize}[leftmargin=*]
    \item 
{\em Input}: A relation $D$ of the tuples of schema $R$, where the tuples in $D$ are divided into $m$ partitions $P_1, \ldots, P_m$.
\item {\em Output}: The set $\kw{Ca}(P_i)$ of candidate tuple pairs on each $P_i$.
\end{itemize}



\eat{
\stitle{Our problem setting.}
Much of the literature uses the terms "data partitioning" and "blocking" interchangeably, as they share the same goal but are complementary. 
In this paper, we adhere to the definition provided by~\cite{DeepBlocking} and focus  on the blocking phrase. 

Thus, our focus is on tackling the problem of efficiently blocking tables $\E$ in order to generate 
$\kw{Ca}(\E)$.
Our objective is to develop effective solutions that expedite the blocking procedure.

\eat{
Much of the literatures uses two concepts, data partitioning and blocking,  interchangeably, due to these two 
these two phrase share the same goal but are complementary.
In this paper, we follow the definition of literature~\cite{DeepBlocking} and focus on the blocking phrase.
That is, we consider the problem of blocking  tables $\E$ to produce set of all
pairs of matching entity profiles $\D(\E) = \{ (t, s):t\in \E , s\in \E, t = s\}$..
We seek to develop solutions that speed up the blocking procedure. 
}
}

\stitle{Rule-based blocking.}
We study rule-based blocking in this paper,
due to its efficiency and explainability.
We review a class of matching dependencies (\MDs), originally proposed in~\cite{fan2011dynamic}. \looseness=-1


\etitle{Predicates.}
Predicates over schema $R$ are defined as follows:
\vspace{-0.7ex}
\[ 
    p::= t.A=c\ |\ t.A=s.B\ |\  t.A \approx s.B
\vspace{-0.7ex}
\]
where $t$ and $s$ are tuple variables denoting tuples of $R$, $A$ and $B$ are attributes
of $R$ and $c$ is a constant; 
$t.A = s.B$ and $t.A=c$ compare the equality on \emph{compatible} attribute values, while
$t.A \approx s.B$ 
compares the \emph{similarity} of $t.A$ and $s.B$.
Here any similarity metric can be used as $\approx$, 
\eg q-grams, Jaro distance or
edit distance, such that $t.A \approx s.B$  is true
if $t.A$ and $s.B$ are “similar” enough w.r.t. a predefined threshold.
In particular, $t.\eid = s.\eid$ says that $t$ and $s$
\revise{are a potential match} \looseness=-1


\etitle{Rules.}
A (bi-variable) {\em matching dependency} (\MD) over $R$ is:
\vspace{-0.7ex}
\[\varphi = X \ra l,
\vspace{-0.7ex}
\]
where  $X$ is a conjunction of predicates over $R$
with two tuple variables $t$ and $s$, and $l$ is
$t.\eid = s.\eid$.
We refer to $X$ as the {\em precondition}
of $\varphi$, and $l$ as the {\em consequence} of $\varphi$, respectively.


\begin{example}\label{example:2}
Consider an example from a (simplified)  e-commence database with self-explained schema
\kw{Products}(\kw{eid}, \kw{pno}, \kw{pname}, \kw{price}, \kw{sname} (store name), \kw{description}, \kw{color}, \kw{saddress} (store address)).
Below are three examples \MDs over \kw{Products}, where the rule in Example~\ref{example:1} can be written as $\varphi_1$.

\sstab
(1) $\varphi_1:  t.\kw{color} = s.\kw{color}  \land t.\kw{price} = s.\kw{price} \land t.\kw{sname} = s.\kw{sname} \land t.\kw{pname} \approx_\kw{ED} s.\kw{pname} \to t.\kw{eid} = s.\kw{eid}$,
where $\approx_\kw{ED}$ measures the 
 edit distance.
\revise{As stated before, $\varphi_1$ identifies two products, by their
colors, prices, product names and stores. }\looseness=-1

\sstab
(2) $\varphi_2:  t.\kw{sname} = s.\kw{sname} \land t.\kw{description} \approx_\kw{JD} s.\kw{description} \allowbreak \to t.\kw{eid} = s.\kw{eid}$,
where $\approx_\kw{JD}$ measures the 
 Jaccard distance.
 The \MD says that if products are sold in the store and have a similar description, then they are likely to be identified.

\sstab 
(3) $\varphi_3: t.\kw{saddress} \approx_\kw{ED} s.\kw{saddress} \land t.\kw{description} \approx_\kw{JD} s.\kw{des}$-$\kw{cription} \allowbreak  \to t.\kw{eid} = s.\kw{eid}$.
%where $\approx_{EU}$ measures the similarity based on the Euclidean distance. 
It gives another condition for identifying two potential products,
\ie the two products with similar descriptions are sold from stores with similar addresses.
\end{example}
\looseness=-1

\vspace{-0.6ex}
\etitle{Semantics}. 
A {\em valuation} of tuple variables of an \MD
$\varphi$ in $D$, or simply
{\em a valuation of $\varphi$},
is a mapping $h$ that instantiates the two variables $t$ and $s$ with
tuples in $D$.
A valuation $h$ {\em satisfies} a predicate $p$ over $R$,
written as $h \models p$, if the following is
satisfied: (1) if $p$ is $t.A = c$ or  $t.A = s.B$, then it is interpreted
as in tuple relational calculus following the standard
semantics of first-order logic \cite{AbHuVi1995};
and (2) if $p$ is $t.A \approx s.B$, then $h(t).A \approx h(s).B$
returns true.
Given a conjunction $X$ of predicates, we say $h \models X$ if for
{\em all} predicates $p$ in $X$, $h \models p$.


\etitle{Blocking.}
\revise{Rule-based blocking 
%methods~\cite{dedoop,dis-dup,Falcon,Corleone,rules-blocking} often 
employs a set  $\Delta$ of \MDs.}
Given a partition $P$,
a pair $(t_1, t_2) \in P \times P$ is in $\kw{Ca}(P)$ \emph{iff}
there exists an \MD $\varphi: X \ra l$ in $\Delta$ 
such that the valuation $h(t_1, t_2)$ of $\varphi$ that instantiates variables $t$ and $s$ with tuples $t_1$ and $t_2$ satisfies the precondition of $\varphi$;
we call such  $\varphi$ as a \emph{witness} at $(t_1, t_2)$,
since it indicates that $(t_1, t_2)$ is a potential match.
If there exists no such witness at $(t_1, t_2)$,
$(t_1, t_2)$ will be filtered.  \looseness=-1


\begin{example}\label{example:3}
%\warn{Give a toy relation $D$ and  apply \MDs}
Continuing with Example~\ref{example:2},
consider the relation $D$ in Table~\ref{tab:products}.
Consider a valuation $h(t_1, t_4)$ that instantiates variables $t$ and $s$ with tuples $t_1$ and $t_4$ in $D$.
Since $h(t_1, t_4)$ satisfies the precondition of $\varphi_1$, $\varphi_1$ is a witness at $(t_1, t_4)$.
Similarly, one can verify that $\varphi_1$ is not a witness at $(t_2, t_3)$
since $h(t_2, t_3) \not \models t.\kw{price} = s.\kw{price}$ (due to value missing).
\eat{As an example, consider \MDs: $\varphi_1$ and $\varphi_2$.
Our goal is to identify potential matches between pairs of math in the dataset based on a self-explained schema (\kw{Products(pname, price, sname, desc, color)} as shown in Table~\ref{tab:products}).
We have three pairs of valuations: ($t_1$.\kw{eid} =$t_4$.\kw{eid}), ($t_4$.\kw{eid} =$t_5$.\kw{eid}), and ($t_2$.\kw{eid}= $t_3$.\kw{eid}). 
The first two satisfy $\varphi_1$, while the last one satisfies $\varphi_2$. }
\end{example}

\etitle{Discovery of \MDs.}
As noted in~\cite{REE-discovery, topk},
\MDs can be considered as a special
case of entity enhancing rules (\REEs).
Algorithms are in place for
discovering \REEs, \eg~\cite{REE-discovery, topk}.
We can readily \revise{apply} these algorithms for discovering \MDs. 

\begin{table}[]
    \begin{center}
    \caption{Summary of Frequently Used Notations}
    \centering
    %\scriptsize
    \footnotesize
    \begin{tabular}{|c|c|}\hline
        \textbf{Notations} &  \textbf{Definition} \\\hline
        $R$  & A relation schema $(\eid, A_1, \dotsc, A_n)$  \\\hline
      $D / P  $ & A set of tuples / a partition of $D$ \\\hline 
      $m$ & The number of data partitions of $D$ \\\hline 
      $\kw{Ca}(P)$ & A set of potential matches  from $P$ \\\hline  
      $\varphi / \Delta$ & A matching dependency (\MD) / a set of \MDs \\\hline  
      $p / X$ & A predicate / the precondition of an \MD \\\hline  
      $h$ and $h(t_1, t_2)$ & \makecell{A valuation of $\varphi$ that instantiates variables  $t$  \\ and $s$  with tuples $t_1$ and $t_2$;
      $\varphi$ is a witness at \\  $(t_1, t_2)$  if $h$ satisfies  the precondition of $\varphi$ } \\\hline  
      $\T/N/\rho$ & An execution plan (tree) / a node /  a path of $\T$ \\\hline  
      $e/\kw{score}(e)$ & An edge $(N_1, N_2)$ of $\T$ / the score of $e$ \\\hline  
      $\P$ &  The set of predicates in $\Delta$ \\\hline
      \makecell{$\kw{cost}(p, D)$ \\ ($\hat{\kw{cost}}(p, D)$)} &  The (estimated) evaluation cost of $p$ on $D$ \\\hline
      %$\N$ &  A shallow feed-forward neural network \\\hline
      $\kw{sp}(p, D)$ &  The probability of $p$ being satisfied on $D$ \\\hline
      $\kw{wp}(p, D)$ &  The probability of $\varphi$ being a witness \\\hline
      $n_t$/$n_w$ &  The size of intervals / the size of window \\\hline
      %$M$ &  The number of GPUs \\\hline
    \end{tabular}
    \label{tab:notation}
    \end{center}
\vspace{-4ex}
\end{table}


\eat{
we focus on the following
kind of matching rules:
\begin{equation}
l_1 \land l_2 \land ...  l_n \to l
\end{equation}
where $l, l_1,...,l_n$ are one of the following predicates
$\R(e), e.A = C, .$

Here (1) l; l1; : : : ; ln are one of the following predicates
%R(t); t:A = c; t:A = s:B; t:A ≈ t:B; 
}

\eat{
%To tackle ER's inherently quadratic complexity, 
Blocking methods trade slightly lower effectiveness
for significantly higher efficiency. 
It takes as input the 
entity collection $\E$ and yields a set of blocks $\B$.
Its goal is to reduce the number of performed comparisons
while missing as few matches as possible.
To this end, 
it clusters potentially matching entities in common blocks and exclusively
compares entity profiles that co-occur in at least one block.
Formally, a blocking scheme should achieve a good balance between these two competing objectives as expressed through the following measures.

\begin{itemize}
    \item Pair Completeness~(PC) estimating the portion of the detectable duplicates in $\B$ with respect to those in $\E$: $PC(\B) = \frac{|\D(\B)|}{|\D(\E)|} \in [0,1]$.
    \item Reduction Ratio~(RR) measures the reduction in the number of pairwise comparisons in $\B$ with respect to the brute-force approach: $RR(\B, \E) = 1-\frac{||\B||}{||\D||} \in [0,1]$.
\end{itemize}
where the number of  set of detectable duplicates in $\B$ is denoted as $|\D(\B)|$,
while  $|\D(\E)|$ stands for the number of all existing duplicates. 
Cardinality $||\B||$ and $||\D||$ refer to as the number of comparisons in $\B$ and $\D$, respectively.

Previous parallel ER solutions based on inter-block task parallelism.
They build up on either redundancy-free blocking~\cite{dedoop,fellegi1969theory}
or  Redundancy-positive blocking~\cite{dis-dup,DraisbachN11,YanLKG07}.
The former assigns every entity to a single block, thus having a  tradeoff between block quality and block size.
The latter places every entity into multiple blocks,
yielding overlapping blocks, thus yielding additional computation and data transfer overhead.
There is no perfect solution to inter-block task parallelism ER solutions.
In contrast, we show that \Hyper achieves optimality for both PC and PR, 
due to our hybrid parallel execution model.
}

\stitle{GPU hardware.}
GPUs were initially designed as specialized processors to accelerate graphics rendering. However, driven by the increasing demand for real-time/high-performance computation, GPUs have evolved into general processors for more workloads. %than just graphics rendering. 
\revise{Compared with CPUs, GPUs offer unique benefits.} \looseness=-1


Firstly, GPUs provide massive parallelism
by utilizing thousands of CUDA cores, 
which can perform computation
at a throughput %several orders of magnitude 
much higher
than CPUs.
%For instance, each Nvidia GeForce RTX 3090 Ti GPU packs
%10752 cores packed into multiple streaming multiprocessors~(SM).
A GPU has multiple streaming multiprocessors (SM),
where 
each SM accommodates multiple processing units. 
This organization leads to a hierarchical parallel model: 
each CUDA kernel includes groups of threads, called thread blocks~(TBs). 
In each TB, subgroups of 32 threads, called warps, are executed simultaneously. 
%Each core  work at  1920 MHz in the manner of Single instruction, multiple threads~(SIMT).
%At a high level, to arrange these cores, GPU splits them into thread grids~(TG) of thread blocks~(TB),
%where each TB contains multiple threads and each TG contain multiple TBs.
\looseness=-1


Secondly,
GPUs are equipped with wider/faster memory interfaces, enabling quick access to large  data. Using tightly integrated
high-bandwidth memory technologies, GPUs provide 
a device memory with bandwidth approaching 1 TB/sec.
This is particularly useful for tasks with data-intensive operations.
%such as image and video processing. 
\looseness=-1

Finally, GPUs offer a variety
of features, like programmable on-chip shared memory, similar to a CPU cache, with a peak bandwidth of
several TB/sec, thread and warp synchronization primitives, and techniques to overlap computation with I/O. 
%These benefits lead to new opportunities for optimizations.
\looseness=-1


